On Approximation Guarantees for Greedy Low Rank Optimization

We provide new approximation guarantees for greedy low rank matrix estimation under standard assumptions of restricted strong convexity and smoothness. Our novel analysis also uncovers previously unknown connections between the low rank estimation and combinatorial optimization, so much so that our bounds are reminiscent of corresponding approximation bounds in submodular maximization. Additionally, we also provide statistical recovery guarantees. Finally, we present empirical comparison of greedy estimation with established baselines on two important real-world problems.

==> distributed.tex <==
\section{Distributed Greedy}
The distributed greedy algorithm is illustrated in Algorithm~\ref{algo:distributedgreedy}. We assume the sets $\cU$ and $\cV$ are partitioned into $l$ subsets each.



\begin{algorithm}[h]
\caption{\textsc{DistributedGreedy}($l$, $k$, $\{\cU_j\}$, $\{\cV_j\}$ )}
\label{algo:distributedgreedy}
\begin{algorithmic}[1]
%\STATE Input: sparsity $k$, number of parallel solvers $l$, partition $\{\sfp_i\} $ of $[p]$
%\STATE $\sfS_i \leftarrow $ \func($\sfp_i$, $k$) $\forall i \in [m]$
\STATE Input: sparsity $k$, number of parallel solvers $l$, partitions $\{\cU_j\}$, $\{\cV_j\}$ of the vector atomic sets
\STATE $\sfG_i \leftarrow $ \func($\cU_i$, $\cV_i$ $k$) $\forall i \in [l]$
\STATE $\sfG \leftarrow$ \func($\cup_i \cU[\sfG_i$], $\cup_i \cV[\sfG_i$], $k$)
\STATE $\sfG_{\text{max}} \leftarrow \arg\max_{\sfG_j} f(\sfG_j) $
\STATE return $\arg\max f(\sfG), f( \sfG_\text{max})$
\end{algorithmic}
\end{algorithm}

We next prove the subadditivity bound. 
\begin{theorem}
\label{thm:RSCsubadd}
Say the function $ l(\cdot):\bbR^{n\times d} \rightarrow \bbR$ is $m$ strongly concave and $L$-smooth over all $\bx$ supported on $\sfS$. Then, the subadditivity ratio can be lower bounded as : 
\begin{equation}
\kappa_\sfS \geq  \frac{m}{M}
\end{equation}
\end{theorem}

To prove Theorem~\ref{thm:RSCsubadd}, we make use of the following two results.

Note: I think smoothness is required over entire $\sfS$ as opposed to weak submod case. 
\begin{lemma}
\label{lem:rsclem1}
For a support set $\sfL$, $f(\sfS) - f(\emptyset) \geq \frac{1}{2 M} \| P_{\bU_\sfS} \nabla l(\mathbf{0}) P_{\bV_\sfS} \|_F^2$
\end{lemma}
\begin{proof}
Let $\bV = \bU_\sfS \bH \bV_\sfS$ where $\bH$ is an arbitrary $|\sfS| \times |\sfS|$ matrix. By definition of $\bB^{(\sfS)}$, $l(\bB^{(\sfS)}) \geq l(\bV)$. Using the smoothness of $l(\cdot)$,

\begin{align*}
l(\bB^{(\sfS)})  - l(\mathbf{0}) & \geq l(\bV) - l(\mathbf{0}) \\
&\geq \inprod{\nabla l(\mathbf{0})}{\bV} - \frac{M}{2} \| \bV\|_F^2
\end{align*}

Using $\bV = P_{\bU_\sfS} \nabla l(\mathbf{0}) P_{\bV_\sfS}$, we get the desired result.  

\end{proof}
\begin{lemma}
\label{lem:rsclem2}
For any support set $\sfS$,  $f(\sfS) \leq \frac{1}{2 m} \| P_{\bU_\sfS} \nabla l(\mathbf{0}) P_{\bV_\sfS} \|_F^2$
\end{lemma}
\begin{proof}
By strong concavity, 
\begin{align*}
l(\bB^{(\sfS)}) - l(0) & \leq \inprod{ \nabla l(0) }{\bB^{(\sfS)} } - m/2 ||\bB^{(\sfS)}||_F^2 \\
& \leq \max_{\bV} \inprod{ \nabla l(0) }{ \bV)}  - m/2 \| \bV \|_F^2,
\end{align*}

where $\bV $ has column space in $\Sspan(\bU_\sfS)$  and row space in $\Sspan(\bV_\sfS)$. Optimizing the RHS over $\bV$ gives the desired result. 
\end{proof}

